From Gap-ETH to FPT-Inapproximability: Clique, Dominating Set, and More

We consider questions that arise from the intersection between the areas of polynomial-time approximation algorithms, subexponential-time algorithms, and fixed-parameter tractable algorithms. The questions, which have been asked several times (e.g., [Marx08, FGMS12, DF13]), are whether there is a non-trivial FPT-approximation algorithm for the Maximum Clique (Clique) and Minimum Dominating Set (DomSet) problems parameterized by the size of the optimal solution. In particular, letting $\text{OPT}$ be the optimum and $N$ be the size of the input, is there an algorithm that runs in $t(\text{OPT})\text{poly}(N)$ time and outputs a solution of size $f(\text{OPT})$, for any functions $t$ and $f$ that are independent of $N$ (for Clique, we want $f(\text{OPT})=\omega(1)$)? In this paper, we show that both Clique and DomSet admit no non-trivial FPT-approximation algorithm, i.e., there is no $o(\text{OPT})$-FPT-approximation algorithm for Clique and no $f(\text{OPT})$-FPT-approximation algorithm for DomSet, for any function $f$ (e.g., this holds even if $f$ is the Ackermann function). In fact, our results imply something even stronger: The best way to solve Clique and DomSet, even approximately, is to essentially enumerate all possibilities. Our results hold under the Gap Exponential Time Hypothesis (Gap-ETH) [Dinur16, MR16], which states that no $2^{o(n)}$-time algorithm can distinguish between a satisfiable 3SAT formula and one which is not even $(1 - \epsilon)$-satisfiable for some constant $\epsilon > 0$. Besides Clique and DomSet, we also rule out non-trivial FPT-approximation for Maximum Balanced Biclique, Maximum Subgraphs with Hereditary Properties, and Maximum Induced Matching in bipartite graphs. Additionally, we rule out $k^{o(1)}$-FPT-approximation algorithm for Densest $k$-Subgraph although this ratio does not yet match the trivial $O(k)$-approximation algorithm.

==> prevworks.tex <==
\subsection{Comparing Our Techniques to Previous Works.}

In this section, we compare our results with that of the previous works.
There have been several attempts to rule out FPT-approximation algorithm
for \Clique and \DomSet. See, e.g., \cite{ChitnisHK13,HajiaghayiKK13,KhotS16,ChenL16}. 
Here we discuss the techniques in \cite{HajiaghayiKK13} are similar to ours (note, however, that our techniques are based on the earlier works in \cite{ChenHKX06b,PatrascuW10}).

Hajiaghayi~et~al.~\cite{HajiaghayiKK13} showed the running time lower bound in terms of the optimal solution by reducing / compress the size of the optimal solution. 
Their starting point are the known hardness reduction from \SAT of size $n$ to \Clique \cite{FGLSSxxx} and to \DomSet \cite{Feige98}. 
The authors then reduce the size of the optimal solution by enumerating all the possilbe subsets of size $s$.
For \DomSet, they use the approximation gap from the {\em Label Cover} problem.
For \Clique, they amplify the hardness of approximation later by graph product.
Since there are super constant blow-up during in the first step, their construction gives an instance of size at least $\binom{n}{s}$. 

Our techniques are different from that in \cite{HajiaghayiKK13} for a few reasons. 
Firstly, we apply the techniques in \cite{ChenHKX06b} to reduce the size of the optimal solution and amplifying the approximation hardness at the CSP level.
All the techniques are applied directly to \SAT (which we abstract by a CSP called maxcover) before invoking standard reductions.
Secondly, our gap amplification are done by the randomized graph product (please see \cite{BellareGS98}), thus we obtain a much smaller blow-up. 
For \DomSet, we reduce the size of the optimal solution by simply arbitrary partitioning the variables of the \SAT instance without enumerating all the possible subsets.
This way, our reductions are more efficient than that in \cite{HajiaghayiKK13}.

We remark that as we manipulate the CSP instance, we lose the projection property required in the previous reductions to \DomSet \cite{LundY93,Feige04}.
The key different in our reduction at those in \cite{LundY93,Feige04} are
that we require the {\em hypercube partition system}, which is more robust
than the other partition systems.

